Nearly Optimal Latent State Decoding in Block MDPs

We investigate the problems of model estimation and reward-free learning in episodic Block MDPs. In these MDPs, the decision maker has access to rich observations or contexts generated from a small number of latent states. We are first interested in estimating the latent state decoding function (the mapping from the observations to latent states) based on data generated under a fixed behavior policy. We derive an information-theoretical lower bound on the error rate for estimating this function and present an algorithm approaching this fundamental limit. In turn, our algorithm also provides estimates of all the components of the MDP. We then study the problem of learning near-optimal policies in the reward-free framework. Based on our efficient model estimation algorithm, we show that we can infer a policy converging (as the number of collected samples grows large) to the optimal policy at the best possible rate. Interestingly, our analysis provides necessary and sufficient conditions under which exploiting the block structure yields improvements in the sample complexity for identifying near-optimal policies. When these conditions are met, the sample complexity in the minimax reward-free setting is improved by a multiplicative factor $n$, where $n$ is the number of possible contexts.

==> app_0_changes.tex <==
\section{Possible changes}
How about focusing on the {\bf offline} nature of our problem??

\subsection{Offline Model Estimation}
Many of the model estimation works focus on active model estimation in which the exploration policy is adaptive \cite{Tarbouriech19,Tarbouriech20a}.

However, in batch/offline RL, not much has been done, especially for block MDPs.
Closest works are \cite{duan2018state} and \cite{Azizzadenesheli16a,Azizzadenesheli16b};
\cite{duan2018state} considers {\it soft state aggregation} of uncontrolled Markov chains from a single trajectory that is given (i.e. offline); \cite{Azizzadenesheli16a} does parameter estimation of POMDPs via spectral methods and some optimization {\it per} episode (so it's online, but offline for each trajectory); \cite{Azizzadenesheli16b} takes similar approach for ROMDPs to accurately estimate the clustering function.

\subsection{Offline reward-free RL}

\subsubsection{\cite{xiao2022curse} (Xiao et al., AISTATS'22)}
In offline/batch RL, there are two subproblems: {\it design problem} and {\it policy optimization problem}

The design problem is regarding how the data is collected; this can be done either actively or passively.
Active data collection has been studied especially in reward-free exploration \cite{jin2020reward,kaufmann2021adaptive,zhang2020nearly}.
However, it may be more desirable to use passive data collection strategy for applications such as healthcare, autonomous driving...etc, where active data collection is either impractical or dangerous \cite{levine2020offline}.

For the guarantees, they make the following assumption:
\begin{assumption}[Section 2 of \cite{xiao2022curse}]
	Assume that the initial state is randomly chosen from a distribution that is supported on the whole of the state space.
\end{assumption}

With memoryless logging policy, they prove the following:
\begin{theorem}[Theorem 2 of \cite{xiao2022curse}]
	Any $(\varepsilon, \delta)$-sound algorithm needs at least $\Omega(A^{\min(S-1,H)} \log(1/\delta) / \varepsilon^2)$ episodes.
\end{theorem}
\begin{proof}
	Very similar to ours! Constructs a hard instance of MDP inspired from the combination lock problem \cite{Whitehead91}, and uses Bretagnolle-Huber inequality.
\end{proof}
\begin{corollary}[Corollary 3 of \cite{xiao2022curse}]
	If the logging policy is not uniform, then the sample complexity in above statement increases i.e. the uniform policy is the best logging policy, for memoryless passive data collection.
\end{corollary}
\begin{enumerate}
	\item Maybe we only need to consider uniform policy? We might not even need (iv) of Assumption \ref{assumption:regularity}.
	
	\item We can compare our sample complexity lower bound (Theorem \ref{thm:lower-boundSC1})! We can argue that in our more restricted setting ($\eta$-regularity), we still obtain a similar lower bound with the same dependency on $\varepsilon$.
	Moreover, the quantity $\Lambda(\Phi)$, although does not depend on the number of contexts $n$, still can be exponential (or worse) in the number of latent states $S$ and actions $A$.
\end{enumerate}

They then prove that the plug-in estimator (the ones that we use) achieves somewhat matching upper bound:
\begin{theorem}[Theorem 5 and Remark 2 of \cite{xiao2022curse}]
	When the logging policy is uniform, then the plug-in algorithm finds an $O(\varepsilon)$ optimal policy with $\tilde{O}(S^3 A^{\min(H, S) + 2} \log(1/\delta) / \varepsilon^2)$ episodes.
\end{theorem}

{\color{red} We should also use the terminology ``batch policy optimization in reward-free setting'' and compare our results with this paper, for reward-free RL part. This setting has been considered in the next paper:}



\subsubsection{\cite{yin2021optimal} (Yin \& Wang, NeurIPS'21)}
Their prime object of study is {\it uniform off-policy evaluation (OPE)}, from which they argue several theoretical results for offline learning in general.

To do that, they impose the following assumption:
\begin{assumption}[Assumption 2.4 of \cite{yin2021optimal}]
	Logging policy $\mu$ satisfies $\min_s d^\mu(s) > 0$ for any ``accessible'' state $s$ (i.e. there exists a policy $\pi \in \Pi$ s.t. $d^\pi(s) > 0$).
	Moreover, $d_m = \min_{s,a} \left\{ d^\mu(s, a) | d^\mu(s, a) > 0 \right\}$ is well-defined, where $d^\pi(s, a) := \frac{1}{H} \sum_{h=1}^H \PP[s_h = s | s_1, \pi] \pi_h(a | s)$.
\end{assumption}

Now the result for offline learning:
\begin{corollary}[Corollary 4.2 of \cite{yin2021optimal}]
	If $\epsilon_{opt} \leq \sqrt{H/S}$ and that $\sup_t \lVert \hat{V}_t^{\hat{\pi}} - \hat{V}_t^{\hat{\pi}^*} \rVert_\infty \leq \epsilon_{opt}$, when $T > O(\iota / d_m)$, then w.p. $1 - \delta$, the following inequality holds elementwise:
	\begin{equation*}
		V_1^\star - V_1^{\hat{\pi}}
		\leq \left( C \left[ \sqrt{\frac{H \iota}{T d_m}} + \frac{H^{3/2} S^{1/2} \iota}{T d_m} \right] + \epsilon_{opt} \right)
		\bm{1}
	\end{equation*}
\end{corollary}

They then define the offline reward-free learning:
\begin{definition}[Definition 5.2 of \cite{yin2021optimal}]
	Given a offline exploration dataset, use it to output $\epsilon$-optimal policy for any given rewards?
\end{definition}
\begin{theorem}[Theorem 5.4 of \cite{yin2021optimal}]
	We're given an offline exploration dataset $\cD' = \left\{ (s_h^{(t)}, a_h^{(t)}) \right\}_{h \in [H], t\in [T]}$ by some fixed exploration policy $\mu$.
	For any reward $r$ denote the corresponding MDP $\cM = (\cS, \cA, P, r, H, d_1)$ ($d_1$ is the init state distribution).
	Denote $\iota = \log(HSA / \delta)$ and $\hat{\pi}_\cM^\star = \argmax_\pi \hat{V}_{1,M}^\pi$ (for any given reward $r$, but we omit the dependency for simplicity)
	Then for $T > O(S \iota / d_m)$, w.p. $1 - \delta$ we have that
	\begin{equation*}
		\sup_r \left\lVert V_{1,M}^\star - V_{1,M}^{\hat{\pi}_\cM^\star} \right\rVert_\infty \leq O\left( \sqrt{\frac{H S \iota}{T d_m}} + \frac{H S \iota}{T d_m} \right)
	\end{equation*}
	i.e. $T = \tilde{O}(H S / d_m \epsilon^2)$.
\end{theorem}

One of their contributions is that they've provided the {\bf first} statistical guarantees of reward-free learning in {\it offline} setting; all previous works \cite{jin2020reward,kaufmann2021adaptive,Menard21,zhang2020nearly} consider online reward-free RL.



\subsubsection{\cite{ren2021nearly} (Ren et al., NeurIPS'21)}
They start with two assumptions:
\begin{assumption}
	$\sum_h r_h \leq 1$ a.s.
\end{assumption}
\begin{assumption}
	$N(s, a) \geq TH d_m$, where $d_m$ is the minimum reaching probability.
\end{assumption}
\begin{remark}
	With a fixed logging policy $\mu$, we can view $d_m$ as $d_m = \min_{s,a} d^\mu(s, a) \triangleq \frac{1}{H} \sum_{h=1}^H \PP[s_h = s | s_1, \pi] \pi_h(a | s)$.
	This is a stronger assumption than \cite{yin2021optimal}, as this is saying that the exploration should reach every state, regardless of whether it's ``reachable'' or not.
\end{remark}

They then provide a upper bound and minimax lower bound for the OPE:
\begin{theorem}[Theorem 3 of \cite{ren2021nearly}]
	Suppose $T = \tilde{\Omega}(1 / d_m)$.
	Then, w.p. at least $1 - \delta$,
	\begin{equation*}
		\left| v^{\pi^\star} - v^{\hat{\pi}^\star} \right| \leq \sqrt{\frac{\iota}{T d_m}} + \frac{\iota S}{T d_m},
	\end{equation*}
	where $\iota$ is some polylog term and $\hat{v}^\pi$ is the estimation resulting from using the plug-in estimators.
\end{theorem}
\begin{theorem}[Theorem 4 of \cite{ren2021nearly}]
	There exists a pair of MDPs $\cM_1, \cM_2$, and an offline data $\cD$ with $|\cD| = TH$ and minimum visiting probability $d_m$ such that for some absolute constant $c_0$, we have
	\begin{equation*}
		\inf_{\hat{v}^\pi} \max_{i \in \{1, 2\}} \PP_{\cM_i} \left[ \left| v^{\hat{\pi}(\cD)} - v^{\pi^\star} \right| > \frac{c_0}{\sqrt{T d_m}} \right] > 0.25,
	\end{equation*}
	where $\hat{v}^\pi$ is any estimator that takes $\cD$ as input.
\end{theorem}
\begin{remark}
	The assumption that $T = \tilde{\Omega}(1 / d_m)$ is actually very similar to our assumption of $TH = \omega(n)$!
	Both asserts that every state should be explored sufficiently!
\end{remark}
\begin{remark}[Remark in pg. 8 of \cite{ren2021nearly}]
	If $d_m = \Omega(1 / SA)$, which is indeed the case for our setting, then we obtain a sample complexity of $\tilde{O}\left( \frac{SA}{\epsilon^2} + \frac{S^2 A}{\epsilon} \right)$, which matches the best known result for online finite-horizon time-homogeneous setting \cite{zhang2021difficult}.
	Compare with our reward-specific guarantee (Theorem \ref{thm:lower-boundSC2})
\end{remark}
They provide similar results for OPE (Theorem 1, 2 of \cite{ren2021nearly})

Our estimation of $p$ and $q$ are precisely the {\it plug-in estimator} as used in \cite{ren2021nearly} and references therein.
We obtain better statistical guarantees by utilizing the block structures!


==> table_of_notations.tex <==
% !TEX root = numericalexperiments_proof.tex


\section{Table of Notations}
\begin{table}[htbp]
	%\caption{Table of Notations}
	\begin{center}% used the environment to augment the vertical space
		% between the caption and the table
		\small 
		\begin{tabular}{c c p{10cm} }
			\toprule
			%\multicolumn{3}{c}{}\\
			%\multicolumn{3}{c}{\underline{Variables, Sets}}\\
			%\multicolumn{3}{c}{}\\
			%\hline
			\multicolumn{3}{l}{\bf Notations common to all models}\\
			\hline
			$n$ &   & Number of items\\
			$m$ &  &  Number of users \\
			$\set{I}$ & & Set of items\\
			$\set{U}$  & & Set of users\\
			$u_t$& & User requesting recommendation at round $t$\\
			$T$ & & Time horizon\\
			$X_{i u}$ & &  Binary random variable to indicate whether user $u$ likes the item $i$\\
			$\rho = (\rho_{i u })_{i \in \set{I}, u \in \set{U}}$ & & Probability that the user $u$ likes the item $i$\\
			$\pi$ & & Algorithm for sequential item selection\\
			$\Pi$ & & Set of all algorithms for sequential item selection\\
			$i_t^\pi $ & & Item selected at round $t$ under $\pi$ \\
			$ \set{F}^\pi_{t-1}$ & & $\sigma$-algebra generated by $(u_t, (u_s, i_s^\pi, X_{i_s^\pi u_s}), s \le t-1)$\\
			$\overline{n}$& & Term $\EXP[\max_{u \in \set{U}} N_u(T)]$\\
			$\overline{N}$& & Term $ \frac{4 \log(m)}{ \log \left(\frac{m \log (m)}{T} + e\right) } + \frac{e^2T}{m}$ 
			\\ \multicolumn{3}{c}{}\\
			\hline
			%		\multicolumn{3}{c}{\underline{Functions, Operators}}\\
			\multicolumn{3}{l}{\bf Generic notations}\\
			\hline
			$\hat{a}$& & Estimated value of $a$ \\
			$ \sigma(A)$ & & $\sigma$-algebra generated by $A$\\
			$\kl(p, q)$& &  Kullback–Leibler divergence from Bernoulli random variable with parameter $p$ to that with parameter $q$\\
			$ \gtrsim$ & & We write $a\gtrsim b$ if $\lim\inf_{T\to\infty}a/b\ge 1$
			\\ \bottomrule
		\end{tabular}
		\normalsize
	\end{center}
	\label{tab:TableOfNotationsGeneral}
	\caption{Table of notations common to all models}
\end{table}


\begin{table}[htbp]
	%\caption{Table of Notations}
	\begin{center}% used the environment to augment the vertical space
		% between the caption and the table
		\small 
		\begin{tabular}{c c p{10cm} }
			\toprule
			%\multicolumn{3}{c}{}\\
			%\multicolumn{3}{c}{\underline{Variables, Sets}}\\
			%\multicolumn{3}{c}{}\\
			%\hline
			\multicolumn{3}{l}{\bf Model A: Clustered items and statistically identical users}\\
			\hline
			$\set{I}_k$ & & Set of items in the item cluster $k$\\
			$\alpha = ( \alpha_k)_{k \in [K]}$ & & Probability that an item is assigned to the item cluster $k$\\
			$K$& & Number of item clusters\\
			$\Delta$& & Minimum difference between the success rates of items in optimal cluster and of items in sub-optimal cluster\\
			$p = (p_k)_{k \in [K]}$ & &  Probability that the user likes the item $i \in \set{I}_k$\\
			 $R^\pi(T)$ & & Regret of an algorithm $\pi$ \\
			$ \Delta_k$ & & Term $p_1 - p_k$\\
			$\phi(k, m, p)$ & & Term $ \frac{1 - e^{-m \gamma(p_1, p_k)}}{ 8(1 - e^{-\gamma(p_1, p_k)})}$  
			\\
			$\gamma(p, q)$ & & Term $ \kl(p,q) + \kl(q, p)$ \\
			$ \eta$& & Term $\min_k p_k (1 - p_k)$\\
			$\set{S}$ & & Set of initially sampled items \\
			$\set{V}$ & & Set of items believed to be in the best cluster
			\\ \bottomrule
		\end{tabular}
		\normalsize
	\end{center}
	\label{tab:TableOfNotationsA}
	\caption{Table of notations: Model A}
\end{table}



\begin{table}[htbp]
	%\caption{Table of Notations}
	\begin{center}% used the environment to augment the vertical space
		% between the caption and the table
		\small 
		\begin{tabular}{c c p{10cm} }
			\toprule
			%\multicolumn{3}{c}{}\\
			%\multicolumn{3}{c}{\underline{Variables, Sets}}\\
			%\multicolumn{3}{c}{}\\
			%\hline
			\multicolumn{3}{l}{\bf Model B: Unclustered items and statistically identical users}\\
			\hline
			$\zeta$ & & Distribution over $[0,1]$\\
			$\mu_x$ & & Term $ \inf\{\gamma \in [0, 1] : \Pr[\rho_i \le \gamma] \ge x\}$\\
			$\varepsilon$ & & Constant  that specifies the $\varepsilon$-best items\\
			$R^\pi_\varepsilon(T)$ & & Satisficing regret of algorithm $\pi$ with a given $\varepsilon>0$\\
			$C$ & & Constant that regularizes the distribution $\zeta(\mu)$\\
			$\set{S}$ & & Set of initially sampled items \\
			$\set{V}$ & & Set of items believed to be in the best cluster
			\\ \bottomrule
		\end{tabular}
		\normalsize
	\end{center}
	\label{tab:TableOfNotationsB}
	\caption{Table of notations: Model B}
\end{table}

\begin{table}[htbp]
	%\caption{Table of Notations}
	\begin{center}% used the environment to augment the vertical space
		% between the caption and the table
		\small 
		\begin{tabular}{c c p{10cm} }
			\toprule
			%\multicolumn{3}{c}{}\\
			%\multicolumn{3}{c}{\underline{Variables, Sets}}\\
			%\multicolumn{3}{c}{}\\
			%\hline
			\multicolumn{3}{l}{\bf Model C: Clustered items and clustered users}\\
			\hline
			$\set{I}_k$ & & Set of items in the item cluster $k$\\
			$\alpha = ( \alpha_k)_{k \in [K]}$ & & Probability that an item is assigned to the item cluster $k$\\
			$\set{U}_\ell$& & Set of users in the user cluster $\ell$\\
			$\beta = ( \beta_\ell)_{\ell \in [L]}$ & & Probability that a user is assigned to the user cluster $\ell$\\
			$K$& & Number of item clusters\\
			$L$ & &  Number of user clusters\\
			$p = (p_{k \ell})_{k \in [K], \ell \in [L]}$& & Probability that the user $u$ likes the item $i$ such that $i \in \set{I}_k$ and $u \in \set{U}_\ell$\\
			$ k_\ell^\star$ & & Term $ \arg \max_k p_{k \ell}$\\ 
			$ \Delta_{k \ell}$ & & Term $p_{k_\ell^\star \ell} - p_{k \ell}$\\
			$\Delta$& & Minimum difference between the success rates of items in optimal cluster and of items in sub-optimal cluster\\
			$\delta_\ell$ & & Term $ \min_{k:\Delta_{k\ell}>0} \Delta_{k\ell}$\\
			$\phi(k,\ell,m,p) $ & & Term $ \frac{1- e^{-m \gamma(p_{k^\star_\ell\ell},p_{k\ell})}}{ 8\left( 1- e^{-\gamma(p_{k^\star_\ell\ell},p_{k\ell})}\right)}$\\
			$\psi(\ell, k, T, m, p)$ & & Term $ \frac{1 - e^{ - \frac{T}{m}\gamma(p_{k_\ell^\star}, p_k) }}{8\left( 1 - e^{ - \gamma(p_{k_\ell^\star}, p_k) }\right)}$\\
			${\cal L}_{\perp}$& & Set $\{ (\ell,\ell')\in [L]^2: p_{k_\ell^\star \ell}\neq p_{k_{\ell'}^\star\ell'}\}$\\
			${\cal L}^{\perp}(\ell)$& & Set $\{ \ell'\neq \ell: k_\ell^\star\neq k_{\ell'}^\star, p_{k_\ell^\star\ell}=p_{k_\ell^\star\ell'}\}$\\
			$R_u^\pi(N)$ & & Accumulated expected regret under $\pi$ for user $u$ when the user has arrived $N$ times\\
			$R^\pi(T)$ & & Regret of an algorithm $\pi$\\
			$\set{S}$ & & Set of initially sampled items\\
			$\set{U}_0$& & Set of initially sampled users\\
			$\set{U}^\star$ & & Set of $(\log T)^2$  users in $\set{U}_0$ who have been arrived the most\\
			$\set{L}(u_t)$& & Upper Condifence Set of the user $u_t$\\
			 $\sigma_\ell$ 	& &Permutation of $[K]$ such that $p_{\sigma_\ell(1)\ell}>p_{\sigma_\ell(2)\ell}\ge \dots \ge p_{\sigma_\ell(K)\ell}$ \\
			$\mathcal{R}_\ell$ & & Set $\left\{r\in [L]: {k_\ell^\star} \neq {k_r^\star}\right\}$\\
			 $\mathcal{S}_{\ell r}$ & & Set $ \{k \in [K] : p_{k\ell} \neq p_{kr}\}$ \\
			$y_{\ell r}$& &  Term $\min_{k\in \mathcal{S}_{\ell r}}|p_{k \ell}-p_{kr}|$\\
			 $\delta$  & & Term $\min_\ell (p_{\sigma_\ell(1)\ell}-p_{\sigma_\ell(2)\ell})$\\
			 $ \epsilon$& & Term $ K\sqrt{\frac{8Km}{t} \log\frac{t}{m}}$ (Updated only when the user clustering is executed)
			\\ \bottomrule
		\end{tabular}
		\normalsize
	\end{center}
	\label{tab:TableOfNotationsC}
	\caption{Table of notations: Model C}
\end{table}


